Two-Step Online Trajectory Planning of a Quadcopter in Indoor Environments with Obstacles

This paper presents a two-step algorithm for online trajectory planning in indoor environments with unknown obstacles. In the first step, sampling-based path planning techniques such as the optimal Rapidly exploring Random Tree (RRT*) algorithm and the Line-of-Sight (LOS) algorithm are employed to generate a collision-free path consisting of multiple waypoints. Then, in the second step, constrained quadratic programming is utilized to compute a smooth trajectory that passes through all computed waypoints. The main contribution of this work is the development of a flexible trajectory planning framework that can detect changes in the environment, such as new obstacles, and compute alternative trajectories in real time. The proposed algorithm actively considers all changes in the environment and performs the replanning process only on waypoints that are occupied by new obstacles. This helps to reduce the computation time and realize the proposed approach in real time. The feasibility of the proposed algorithm is evaluated using the Intel Aero Ready-to-Fly (RTF) quadcopter in simulation and in a real-world experiment.

==> setup_and_model.tex <==
\subsection{Equipment} \label{sec:Equipment}
In this work, the Intel Aero ready-to-fly (RTF) drone, equipped with a front-facing RealSense R200 RGB-D camera, is used. The control functionality of which is fulfilled by two main components, i.e. the Intel Aero compute board and the Intel flight controller board. 
The compute board runs a linux distribution, which allows the appliance of additional middleware, i.e. the Robot Operating System (ROS). The compute board takes care of high level tasks, e.g. communications from/to other PCs as well as handling camera data. 
The flight controller board executes the open source PX4 Autopilot program%\cite{px4 website}
, which handles the low-level tasks, e.g. reading sensor data and control the brushless motors, etc. 

The autopilot program allows the definition of setpoints for position, speed, orientation and angular speed of the drone. In combination with sensor data and estimated states from an extended Kalman filter (EKF)% \cite{link to ekf}
, these setpoints serve as an input for the cascaded trajectory tracking controller% \cite{link to control architecture}
.

Depth data of the RGB-D camera is used to detect unknown obstacles in the flight space.

The online trajectory (re)planning task is accomplished on a PC, also known as ground control station (GCS), which is connected to the UAV via wifi. Also, the computational heavy point cloud processing of the depth camera data is executed on the GCS.

For development and simulations, the open-source simulator Gazebo is used, which offers a connection to ROS and enables software-in-the-loop (SITL) simulation of the employed PX4 flight stack. 
In real-life experiments, the Intel Aero ready-to-fly (RTF) drone is utilized in combination with an OptiTrack motion capture system, which provides a very robust, highly precise pose information of the UAV in real-time.

\begin{figure}
    \centering
    \includegraphics[height=.39\textheight]{graphics/SystemArchitecture_v3.pdf}
    \caption{Overview of the simulation and experiment setup.}
    \label{fig:SystemArchitecture}
\end{figure}

\subsection{Environment and obstacle modelling} \label{sec:Environment}

In this work, the admissible flight space $\mathcal{X}$ is described as a cuboid with maximum lengths in the three cartesian dimensions of the world coordinate frame $\mathcal{I}_W$, see Fig. \ref{fig:FlightEnvironment}. For the sake of simplicity and safety, all obstacles $\mathcal{O}$ are considered to be convex, i.e., cuboids, which are aligned with the world frame $\mathcal{I}_W$. The obstacle free space denoted as $\mathcal{X}_{free}$ is obtained by excluding obstacles from the flight space, i.e. $\mathcal{X}_{free} = \mathcal{X}\setminus\mathcal{O}$. 

\begin{figure}
    \centering
    \includegraphics[height=.2\textheight]{graphics/FlightEnvironment3.pdf}
    \caption{Visualization of the  environment with the flight space $\mathcal{X}$ in gray color and exemplary representation of obstacles $\mathcal{O}$. The obstacles (in red color) are inflated due to safety reasons (in green color).}
    \label{fig:FlightEnvironment}
\end{figure}

%\subsection{Dynamic model} \label{sec:DynamicModel}

%standard quadcopter model without disturbances. Z-X-Y Euler angles, proven to be differentially flat in \cite{mellinger_minsnap_2011} with flat outputs
%\begin{equation}
%    \sigma = \begin{bmatrix}
%      x, y, z, \psi
%    \end{bmatrix}^\mathrm{T}
%\end{equation}
%\begin{figure}
%    \centering
%    \includegraphics[height=.2\textheight]{graphics/UAVwithFrames.pdf}
%    \caption{The reference frames and the flat outputs $\Vec{r}$ and $\psi$.}
%    \label{fig:UAVframes}
%\end{figure}
